Modeling Multivariate Positive-Valued Time Series Using R-INLA

In this paper we describe fast Bayesian statistical analysis of vector positive-valued time series, with application to interesting financial data streams. We discuss a flexible level correlated model (LCM) framework for building hierarchical models for vector positive-valued time series. The LCM allows us to combine marginal gamma distributions for the positive-valued component responses, while accounting for association among the components at a latent level. We use integrated nested Laplace approximation (INLA) for fast approximate Bayesian modeling via the R-INLA package, building custom functions to handle this setup. We use the proposed method to model interdependencies between realized volatility measures from several stock indexes.

==> 06_Empirical_Analysis.tex <==

\section{Interdependence Across Realized Volatility Measures}

Volatility measurement is central to asset pricing, asset allocation, portfolio optimization and risk management. A first attempt to measure volatility using intraday data was made by \cite{parkinson1980extreme} for the estimation of the daily
range. Since then the literature has expanded significantly from the realized volatility of \cite{andersen1998answering} to bipower variation \citep{barndorff2004power}, realized kernels of \cite{barndorff2009realized} and realized covariance matrices \citep{ait2010high,peluso2014bayesian}. As these intraday volatility measures evolved, there has been a natural complementary effort to build adequate models to describe their joint dynamics \citep{engle2006multiple,donelli2021bayesian,cipollini2013semiparametric}.


\subsection{Data description}
The focus of this study is to model three robust intraday volatility measures: realized kernel variance based on parzen kernel ($rk$), bipower variation ($bv$) and realized variance ($rv$) using the different level correlated model specifications for the $30$ index data (as shown in Table~\ref{tab:data}) available on Oxford-Man Institute's Quantitative Finance Realized Library \citep{heber2009oxford}. These volatility measures are based on $5$-min sampling frequency.
The sample period spans from January $2$, $2015$, to December $29$, $2017$.  The number of observations for each stock index is 513. 
\begin{table}[H] 
\begin{center}
\caption{List of assets along with their associated region}
\fontsize{8}{10}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Symbol} & \textbf{Name}                             & \textbf{Region} \\ \hline
.AEX            & AEX index                                 & Netherlands      \\ \hline
.AORD           & All Ordinaries                            & Australia        \\ \hline
.BFX            & Bell 20 Index                             & Belgium          \\ \hline
.BSESN          & S\&P BSE Sensex                           & India            \\ \hline
.BVSP           & BVSP BOVESPA Index                        & United States    \\ \hline
.DJI            & Dow Jones Industrial Average              & United States    \\ \hline
.FCHI           & CAC 40                                    & France           \\ \hline
.FTMIB          & FTSE MIB                                  & Italy            \\ \hline
.FTSE           & FTSE 100                                  & United Kingdom   \\ \hline
.GDAXI          & DAX                                       & Germany          \\ \hline
.GSPTSE         & S\&P/TSX Composite index                  & Canada           \\ \hline
.HSI            & HANG SENG Index                           & Hong Kong        \\ \hline
.IBEX           & IBEX 35 Index                             & United States    \\ \hline
.IXIC           & Nasdaq 100                                & United States    \\ \hline
.KS11           & Korea Composite Stock Price Index (KOSPI) & South Korea      \\ \hline
.KSE            & Karachi SE 100 Index                      & Pakistan         \\ \hline
.MXX            & IPC Mexico                                & Mexico           \\ \hline
.N225           & Nikkei 225                                & Japan            \\ \hline
.NSEI           & NIFTY 50                                  & India            \\ \hline
.OMXC20         & OMX Copenhagen 20 Index                   & Denmark          \\ \hline
.OMXHPI         & OMX Helsinki All Share Index              & Finland          \\ \hline
.OMXSPI         & OMX Stockholm All Share Index             & Sweden           \\ \hline
.OSEAX          & Oslo Exchange All-share Index             & Norway           \\ \hline
.RUT            & Russel 2000                               & United States    \\ \hline
.SMSI           & Madrid General Index                      & Spain            \\ \hline
.SPX            & S\&P 500 Index                            & United States    \\ \hline
.SSEC           & Shanghai Composite Index                  & China            \\ \hline
.SSMI           & Swiss Stock Market Index                  & Switzerland      \\ \hline
.STI            & Straits Times Index                       & Singapore        \\ \hline
.STOXX50E       & EURO STOXX 50                             & Europe           \\ \hline
\end{tabular}
\label{tab:data}
\end{center}
\end{table}

\subsection{Realized Volatility Measures} \label{Data Description}
Let $\{P_{t_{j}}\}$ be a sequence of observed intraday prices of an asset. Consider a time interval $[a,b]$ and the time index $t_j$ for $t_j \in [a,b]$. The time is partitioned into $M$ equidistant points in time $j=1,\dots,M$. At each time point $t_j$, the price of an asset is observed. Then $\{P_{t_{j}}\}_{j=1}^{M}$ is the observed sequence of prices of an asset sampled at frequency $\tau=\frac{b-a}{M-1}$. Hence the intraday returns over the sub-interval $[t_{j-1},t_j)$ is defined as 
$r_{j} = \log(P_{t_j}) - \log(P_{t_{j-1}})$. 
To obtain realized variances at 5-minutes sampling frequency, $\tau = 300$ seconds and similarly for 1-minute sampling frequency, $\tau = 60$ seconds. 
%Let $\{P_{t_{j}}\}$ be a sequence of observed intraday prices of an asset.
%Let $P_t$ be the observed price of an asset for day $t = 1,\dots,n$. Divide each day into fixed $M$ sub-intervals and let $\Delta = \frac{1}{M}$, denote the length of time between the two consecutive observations. To obtain realized variances at 5-minutes sampling frequency, $\Delta = 300$ seconds and similarly for 1-minute sampling frequency, $\Delta = 60$ seconds. Let $\{P_{t-1+j\Delta}\}_{j=1}^{M}$ denote the sequence of observed prices for a day $t$ at the sampling frequency $\Delta = \frac{1}{M}$. It is important for alignment of observed prices to time clock in case of missing observed prices, previous tick method or linear interpolation between adjacent ticks 
%\citep{zivot2007modeling} can be used.
%The $j^{th}$ intraday return for day $t$ is defined as
%\begin{equation}
%    y_{j,t} = \ln P_{t-1+j\Delta} - \ln P_{(t-1)+(j-1)\Delta},
%    \quad j=1,\dots,M.
%    \label{intraday_returns}
%\end{equation}

Let us denote $r_{j,t}$ as the $j^{th}$ intraday return for $t^{th}$ day, for $t=1,\dots,T$. 
%Hence for each day $t$, the realized variance
We define some popular measures of intraday volatility considered in the literature.
Realized Variance ($\text{RV}_{t}$) for the $t^{th}$ day is defined as the cumulative squared sum of the intraday returns $r_{j,t}$, 
\begin{equation}
    \text{RV}_t = \sum_{j=1}^{M} r^2_{j,t}
\end{equation}
and $\sqrt{RV_t}$ is known as the realized volatility. A simple and comprehensible measure, which isolates the variation of the pure price process is the Bipower variation (BPV). It is calculated as the sum of products of absolute values of two consecutive returns,
\begin{equation}
    \text{BPV}_t = \sum_{j=2}^{M} |r_{j,t}| |r_{j-1,t}|.
\end{equation} 

\cite{barndorff2009realized} proposed the realized kernels estimator, which uses kernel methods to combat market microstructure noise. The realized kernel estimator is
\begin{equation}
\begin{aligned}
    \text{RK}_t = \sum_{h= -H}^{H} k\Big(\frac{h}{H+1}\Big) \gamma_h, \quad \text{where}\\
    \gamma_h = \sum_{i=|h|+1}^{n} r_{i,t} r_{i-|h|,t},
\end{aligned}
\end{equation}
where $k(.)$ is the Bartlett kernel function defined as $k(x) = 1-x$. Let the close-to-close log returns for the $t^{th}$ day be denoted by $r_t$, where $r_t =\ln \frac{P_{t}}{P_{t-1}}$, $P_t$ denoting the closing price of the $t^{th}$ day. For each day $t$, consider the $d=3$-dimensional time series composed of realized volatility, realized kernel and bipower variation, $\boldsymbol{y}_t =(\sqrt{RV}_t,\sqrt{RK}_t,\sqrt{BPV}_t )^\prime$, where $t= 1,\dots,\text{T}.$ 
%This data structure will be used for the first two projects; see Sections \ref{Chapter 1} and \ref{Chapter 2}.

%In the third project (see section \ref{Chapter 3}) we study the irregularly spaced time series of financial returns. Let $\{P_{t_{j}}\}$ be a sequence of observed intraday asset prices available at the microseconds level. To account for microstructure noise, we have considered rounding up to one second and using the median price as the aggregated price at 1 second level \citep{barndorff2009realized}. For univariate volatility analysis, we construct irregularly spaced intraday log returns as 
%\begin{equation}\label{Third_Chapter_data}
% r_{t_{j}}= \log(P_{t_j}) - \log(P_{t_{j-1}})   
%\end{equation}
%for multiple stocks. For multivariate analysis, we choose $n$ stocks with similar liquidity. Using the refresh time sampling procedure from \cite{barndorff2011multivariate}, we synchronize the intraday prices of $n$ stocks. Then, we compute the log return matrix after synchronizing the intraday prices. We consider modeling a $N\times n$ matrix of synchronized irregularly spaced log returns, where $N$ is the number of aligned intraday observations on a particular day.

\subsection{Model Specification}\label{Models}
Let $\boldsymbol{y}_{it} = (y_{1,it} ,\ldots,y_{d,it})^\prime$ be a $d$-variate vector of positive-valued volatility measures over time, for $i = 1,\ldots,n$ and $t = 1,\ldots,T$. That is, we observe $d$ components of different volatility measures on $n$ stock market indexes over $T$ regularly spaced time points. Equations (\ref{Eq: Gamma marginal} - \ref{Eq: Gamma Obs Eqn}) simplifies as
\begin{equation} \label{Eq: LCM1}
\begin{aligned}
 &Y_{j,it} | \theta_{j,it}, \tau \sim   Gamma\bigg(\tau, \frac{\theta_{j,it}}{\tau}\bigg) ,\\
 \log(\theta_{j,it}) = \alpha_{j,i} + \beta_{j,t,0} +  &\beta_{1,j} \log (Y^{(d)}_{j,i,t-1}) + \beta_{2,j} \log  (Y^{(w)}_{j,i,t-1})\\
 + \beta_{3,j} & \log (Y^{(m)}_{j,i,t-1})+ \beta_{4,j} \log(1+ J_{j,i,t-1}) + \xi_{j,it}, \\
% &\beta_{j,it,0} = \phi_{j}\beta_{j,i,t-1,0} + w_{j,it}
\end{aligned}
\end{equation}
where $w_{j,it} \sim N(0,\sigma_j^2)$.
%and $\beta_{j,it,0}$ represents the dynamic intercept which is modeled as a random walk. 
Inspired by \cite{corsi2009simple}, we have used the predictors 
$Y^{(d)}_{j,i,t},Y^{(w)}_{j,i,t},Y^{(m)}_{j,i,t}$ in the model, which represents daily level component driven by short-term traders, weekly component driven by the medium-term investors who typically re-balance their positions weekly and the monthly component driven by long-term agents with a characteristic time of one or more months. These components are defined as $Y^{(d)}_{j,i,t} = Y_{j,i,t-1},\quad Y^{(w)}_{j,i,t} = \frac{1}{5} \sum_{j=1}^{5} Y_{j,i,t-j},\quad Y^{(m)}_{j,i,t} = \frac{1}{22} \sum_{j=1}^{22} Y_{j,i,t-j}$ and $J_t = max(RV_t - BPV_t,0)$, which accounts for the jumps in price process \citep{andersen2007roughing}. Here $RV_t$ and $BV_t$ denotes the realized volatility and bipower variation at time $t$. We assume that the level correlated effect $\boldsymbol{\xi} = (\xi_{1,it},\xi_{2,it}) \sim N(\boldsymbol{0},\boldsymbol{\Sigma})$ where 
\begin{equation}\label{Eq: correlation}
\boldsymbol{\Sigma}=\begin{pmatrix}
1/\sigma^2_1 & \rho_{12}/\sigma_1 \sigma_2 & \rho_{13}/\sigma_1 \sigma_3 \\
\rho_{12}/\sigma_1 \sigma_2 & 1/\sigma^2_2 & \rho_{23}/\sigma_2 \sigma_3\\
\rho_{13}/\sigma_1 \sigma_3 & \rho_{23}/\sigma_2 \sigma_3 & 1/\sigma^2_3\\
\end{pmatrix},
\end{equation}

We have considered two different specifications of the model in equation (\ref{Eq: LCM1}) according to the state equation similar to \ref{AR state eq} and \ref{Eq: VAR_state}. Considering the evolution of the states as AR process, we can write the state equation as
\begin{equation}\label{Eq: AR_evolution}
    \beta_{j,t,0} = \phi_{j}\beta_{j,t-1,0} + w_{j,t},
\end{equation}
where $t = 1 \dots T$ and $j = 1 \dots d$ and the error terms $w_{j,t} \sim N(0, W_{j} )$. Assumption of VAR evolution of the states leads to 
\begin{equation}\label{Eq: VAR_evolution}
    \boldsymbol{\beta}_{t,0} = \boldsymbol{\Phi} \boldsymbol{\beta}_{t-1,0} + \boldsymbol{w}_t,
\end{equation}
the state errors $\boldsymbol{w}_t \sim N(\boldsymbol{0},\boldsymbol{W})$. We refer to equation (\ref{Eq: LCM1}) as LCM1, where the intercept vary by component and stocks. We refer to equations (\ref{Eq: LCM1}) and (\ref{Eq: AR_evolution}) as LCM1-AR, whereas equations (\ref{Eq: LCM1}) and (\ref{Eq: VAR_evolution}) is LCM1-VAR. Likewise, we define LCM2 as
\begin{equation} \label{Eq: LCM2}
\begin{aligned}
 Y_{j,it} | \theta_{j,it} \sim  &  \quad Gamma\bigg(\tau, \frac{\tau}{\theta_{j,it}}\bigg) ,\\
 \log(\theta_{j,it}) = \alpha_{j} + \beta_{j,t,0} +  &\beta_{1,j} \log (Y^{(d)}_{j,i,t-1}) + \beta_{2,j} \log  (Y^{(w)}_{j,i,t-1})\\
 + \beta_{3,j} & \log (Y^{(m)}_{j,i,t-1})+ \beta_{4,j} \log(1+ J_{j,i,t-1}) + \xi_{j,it}, \\
%& \beta_{j,it,0} = \beta_{j,i,t-1,0} + w_{j,it}
\end{aligned}
\end{equation}
Similarly, we refer to equations (\ref{Eq: LCM2}) and (\ref{Eq: AR_evolution}) as LCM2-AR, whereas (\ref{Eq: LCM2}) and (\ref{Eq: VAR_evolution}) is LCM2-VAR. The models defined in (\ref{Eq: LCM1}) and (\ref{Eq: LCM2}) can be seen as a dynamic extension of Heterogeneous Autoregressive (HAR) models \citep{corsi2009simple} which takes into account the dependency among the volatility measures. 



\begin{comment}
%\subsection{Bivariate Analysis}
We consider $\boldsymbol{y}_{it} = (\sqrt{rv_{it}}, \sqrt{rk_{it}})^\prime$ be a bivariate response vector of realized semi-variance and realized kernel variance using the Parzen weight function. We fit the models LCM1 and LCM2 using \texttt{R-INLA}. The Kendall's tau correlation coefficient between the realized semi-variance and realized kernel (parzen) is 0.63. Based on DIC, LCM1 is the best model.

\begin{table}[H]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{DIC} & \textbf{WAIC} & \textbf{CPO} & \textbf{MAE} & \textbf{MAPE} & \textbf{RMSE} \\ \hline
LCM1           & -75391.18    & -73353.12     & 2841.60      & 0.30         & 0.37          & 0.45          \\ \hline
LCM2           & -62495.80     & -59405.40     & 11930.13     & 0.26         & 0.32          & 0.41          \\ \hline
\end{tabular}
\end{center}
\caption{Comparison of In-sample model fits}
\end{table}
\end{comment}


\begin{comment}
%\subsection{Trivariate Analysis}
We consider $\boldsymbol{y}_{it} = (\sqrt{rv_{it}},\sqrt{rk_{it}},\sqrt{bv_{it}})^\prime$ be a trivariate response vector of realized semi-variance \cite{barndorff2008measuring}, realized kernel (Parzen) and bipower variation . The $3\times 3$ Kendall's tau correlation matrix of realized semi-variance, realized kernel (Parzen) and bipower variation is given by
\begin{table}[H]
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
    & rv  & rk   & bv   \\ \hline
rv & 1.00 & 0.63 & 0.73 \\ \hline
rk  & 0.63 & 1.00 & 0.70 \\ \hline
bv  & 0.73 & 0.70 & 1.00 \\ \hline
\end{tabular}
\end{center}
\caption{Kendall's tau correlation matrix of realized semi-variance, realized kernel (parzen) and bipower variation}
\end{table}
We fit LCM1 and LCM2 models to this trivariate setup and compare their in-sample fits. We note that based on DIC, LCM2 is the best model.
\begin{table}[H]
\begin{center}
\begin{tabular}{|c|l|c|c|c|c|c|}
\hline
\textbf{Model} & \multicolumn{1}{c|}{\textbf{DIC}} & \textbf{WAIC} & \textbf{CPO} & \textbf{MAE} & \textbf{MAPE} & \textbf{RMSE} \\ \hline
LCM1           & -184596.7                         & -173370.40    & -40196.05    & 0.30         & 0.37          & 0.46          \\ \hline
LCM2           & -206113.5                         & -205294.20    & -56740.18    & 0.25         & 0.30          & 0.39          \\ \hline
\end{tabular}
\end{center}
\caption{Comparison of In-sample model fits}
\end{table}

\end{comment}


\subsection{Results}
The main goal is to model the interdependence between the robust volatility measures across the stock indexes. For this purpose we have fitted the four models as discussed in subsection (\ref{Models}). We have fitted the four models i.e., LCM1-AR, LCM1-VAR, LCM2-AR and LCM2-VAR using \texttt{R-INLA}. We have used the same prior specification as mentioned in subsection (\ref{Prior}).We have explicitly assumed $\tau \sim Gamma(0.01,0.01)$ such that $E[\tau] = 1$ and $Var[\tau]=100$, which is similar to the simulation setup. 

We note that the estimated level correlation among the three volatility measures i.e $\hat{\rho}_{12},\hat{\rho}_{13}$ and $\hat{\rho}_{23}$ are strong and significant, which is as expected. Hence the interdependence among measures is empirically supported by the significant level correlation of all estimated coefficients, a result which can be achieved by LCM estimation. The beta coefficients related to the jump components were not significant in LCM1-VAR and LCM2-VAR. Most of the estimated coefficients are significant in all the four models. The following tables shows the posterior summaries for LCM 1 and LCM2.



\begin{center}
%\fontsize{8}{10}
%\caption{\normalfont Posterior Estimates for LCM1-VAR and LCM1-AR for Stock Market Index Data}\tabularnewline
\footnotesize
\begin{longtable}{|c|c|c|c|c|}\caption{\normalfont Posterior Estimates for LCM1-VAR and LCM1-AR for Stock Market Index Data} \label{Table-LCM1}
\hline
\multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\textbf{LCM1-VAR}} & \multicolumn{2}{c|}{\textbf{LCM1-AR}} \\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\textbf{Posterior Mean}} & \multicolumn{1}{c|}{\textbf{Posterior SD}} & \multicolumn{1}{c|}{\textbf{Posterior Mean}} & \multicolumn{1}{c|}{\textbf{Posterior SD}} \\ \hline
\endfirsthead
\multicolumn{1}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline
\multicolumn{1}{|c|}{} & \multicolumn{2}{c|}{\textbf{LCM1-VAR}} & \multicolumn{2}{c|}{\textbf{LCM1-AR}} \\ \hline
\multicolumn{1}{|c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{Posterior Mean}} & \multicolumn{1}{c|}{\textbf{Posterior SD}}  & \multicolumn{1}{c|}{\textbf{Posterior Mean}} & \multicolumn{1}{c|}{\textbf{Posterior SD}} \\ \hline 
\endhead
\hline \multicolumn{3}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

\textbf{Stock-Index Specific intercept} & & & & \\
$\alpha_{1,1}$ & -1.843 & 0.070 & -4.342 & 0.035 \\
$\alpha_{1,2}$ & -1.987 & 0.073 & -4.667 & 0.037 \\
$\alpha_{1,3}$ & -1.852 & 0.071 & -4.370 & 0.035 \\
$\alpha_{1,4}$ & -1.891 & 0.072 & -4.457 & 0.036 \\
$\alpha_{1,5}$ & -1.881 & 0.072 & -4.445 & 0.036 \\
$\alpha_{1,6}$ & -1.761 & 0.069 & -4.153 & 0.034 \\
$\alpha_{1,7}$ & -2.000 & 0.074 & -4.686 & 0.037 \\
$\alpha_{1,8}$ & -1.803 & 0.070 & -4.252 & 0.035 \\
$\alpha_{1,9}$ & -1.777 & 0.069 & -4.188 & 0.034 \\
$\alpha_{1,10}$ & -1.892 & 0.072 & -4.464 & 0.036 \\
$\alpha_{1,11}$ & -1.814 & 0.070 & -4.272 & 0.035 \\
$\alpha_{1,12}$ & -1.989 & 0.074 & -4.683 & 0.038 \\
$\alpha_{1,13}$ & -1.938 & 0.073 & -4.561 & 0.037 \\
$\alpha_{1,14}$ & -1.750 & 0.069 & -4.133 & 0.034 \\
$\alpha_{1,15}$ & -1.938 & 0.072 & -4.536 & 0.036 \\
$\alpha_{1,16}$ & -1.975 & 0.074 & -4.659 & 0.037 \\
$\alpha_{1,17}$ & -2.050 & 0.073 & -4.697 & 0.037 \\
$\alpha_{1,18}$ & -1.923 & 0.072 & -4.539 & 0.037 \\
$\alpha_{1,19}$ & -1.953 & 0.072 & -4.568 & 0.037 \\
$\alpha_{1,20}$ & -1.905 & 0.072 & -4.484 & 0.036 \\
$\alpha_{1,21}$ & -1.839 & 0.071 & -4.339 & 0.035 \\
$\alpha_{1,22}$ & -1.903 & 0.072 & -4.485 & 0.036 \\
$\alpha_{1,23}$ & -1.925 & 0.072 & -4.530 & 0.036 \\
$\alpha_{1,24}$ & -1.910 & 0.072 & -4.501 & 0.036 \\
$\alpha_{1,25}$ & -1.951 & 0.073 & -4.574 & 0.037 \\
$\alpha_{1,26}$ & -1.762 & 0.069 & -4.157 & 0.034 \\
$\alpha_{1,27}$ & -2.003 & 0.073 & -4.682 & 0.037 \\
$\alpha_{1,28}$ & -1.850 & 0.070 & -4.340 & 0.035 \\
$\alpha_{1,29}$ & -1.868 & 0.071 & -4.411 & 0.036 \\
$\alpha_{1,30}$ & -1.799 & 0.070 & -4.240 & 0.034 \\
$\alpha_{2,1}$ & -2.190 & 0.071 & -4.132 & 0.038 \\
$\alpha_{2,2}$ & -2.228 & 0.071 & -4.175 & 0.038 \\
$\alpha_{2,3}$ & -2.193 & 0.071 & -4.142 & 0.038 \\
$\alpha_{2,4}$ & -2.219 & 0.072 & -4.206 & 0.039 \\
$\alpha_{2,5}$ & -2.225 & 0.072 & -4.209 & 0.039 \\
$\alpha_{2,6}$ & -2.073 & 0.069 & -3.915 & 0.037 \\
$\alpha_{2,7}$ & -2.320 & 0.074 & -4.373 & 0.040 \\
$\alpha_{2,8}$ & -2.136 & 0.070 & -4.033 & 0.038 \\
$\alpha_{2,9}$ & -2.088 & 0.070 & -3.959 & 0.037 \\
$\alpha_{2,10}$ & -2.153 & 0.071 & -4.072 & 0.038 \\
$\alpha_{2,11}$ & -2.121 & 0.070 & -4.014 & 0.037 \\
$\alpha_{2,12}$ & -2.340 & 0.074 & -4.410 & 0.040 \\
$\alpha_{2,13}$ & -2.182 & 0.071 & -4.128 & 0.038 \\
$\alpha_{2,14}$ & -2.059 & 0.069 & -3.896 & 0.037 \\
$\alpha_{2,15}$ & -2.258 & 0.073 & -4.262 & 0.039 \\
$\alpha_{2,16}$ & -2.350 & 0.075 & -4.426 & 0.040 \\
$\alpha_{2,17}$ & -2.224 & 0.071 & -4.170 & 0.038 \\
$\alpha_{2,18}$ & -2.201 & 0.072 & -4.158 & 0.039 \\
$\alpha_{2,19}$ & -2.253 & 0.072 & -4.219 & 0.039 \\
$\alpha_{2,20}$ & -2.229 & 0.073 & -4.223 & 0.039 \\
$\alpha_{2,21}$ & -2.105 & 0.070 & -3.971 & 0.037 \\
$\alpha_{2,22}$ & -2.212 & 0.072 & -4.168 & 0.039 \\
$\alpha_{2,23}$ & -2.241 & 0.072 & -4.222 & 0.039 \\
$\alpha_{2,24}$ & -2.133 & 0.070 & -4.036 & 0.038 \\
$\alpha_{2,25}$ & -2.171 & 0.071 & -4.097 & 0.038 \\
$\alpha_{2,26}$ & -2.089 & 0.069 & -3.938 & 0.037 \\
$\alpha_{2,27}$ & -2.331 & 0.074 & -4.396 & 0.040 \\
$\alpha_{2,28}$ & -2.067 & 0.069 & -3.905 & 0.037 \\
$\alpha_{2,29}$ & -2.211 & 0.072 & -4.192 & 0.039 \\
$\alpha_{2,30}$ & -2.106 & 0.070 & -3.975 & 0.037 \\
$\alpha_{3,1}$ & -1.772 & 0.055 & -3.997 & 0.031 \\
$\alpha_{3,2}$ & -1.844 & 0.056 & -4.141 & 0.032 \\
$\alpha_{3,3}$ & -1.782 & 0.056 & -4.022 & 0.031 \\
$\alpha_{3,4}$ & -1.823 & 0.056 & -4.114 & 0.031 \\
$\alpha_{3,5}$ & -1.826 & 0.057 & -4.131 & 0.032 \\
$\alpha_{3,6}$ & -1.682 & 0.054 & -3.802 & 0.029 \\
$\alpha_{3,7}$ & -1.920 & 0.058 & -4.314 & 0.033 \\
$\alpha_{3,8}$ & -1.732 & 0.055 & -3.910 & 0.030 \\
$\alpha_{3,9}$ & -1.720 & 0.054 & -3.881 & 0.030 \\
$\alpha_{3,10}$ & -1.808 & 0.056 & -4.079 & 0.031 \\
$\alpha_{3,11}$ & -1.736 & 0.055 & -3.916 & 0.030 \\
$\alpha_{3,12}$ & -1.894 & 0.058 & -4.274 & 0.033 \\
$\alpha_{3,13}$ & -1.799 & 0.056 & -4.059 & 0.031 \\
$\alpha_{3,14}$ & -1.676 & 0.054 & -3.788 & 0.029 \\
$\alpha_{3,15}$ & -1.864 & 0.057 & -4.186 & 0.032 \\
$\alpha{3,16}$ & -1.893 & 0.058 & -4.275 & 0.033 \\
$\alpha_{3,17}$ & -1.845 & 0.056 & -4.142 & 0.032 \\
$\alpha_{3,18}$ & -1.822 & 0.056 & -4.110 & 0.031 \\
$\alpha_{3,19}$ & -1.829 & 0.056 & -4.099 & 0.031 \\
$\alpha_{3,20}$ & -1.833 & 0.057 & -4.135 & 0.032 \\
$\alpha_{3,21}$ & -1.743 & 0.055 & -3.931 & 0.030 \\
$\alpha_{3,22}$ & -1.818 & 0.056 & -4.101 & 0.031 \\
$\alpha_{3,23}$ & -1.838 & 0.057 & -4.147 & 0.032 \\
$\alpha_{3,24}$ & -1.801 & 0.056 & -4.070 & 0.031 \\
$\alpha_{3,25}$ & -1.846 & 0.057 & -4.154 & 0.032 \\
$\alpha_{3,26}$ & -1.690 & 0.054 & -3.818 & 0.030 \\
$\alpha_{3,27}$ & -1.929 & 0.058 & -4.328 & 0.033 \\
$\alpha_{3,28}$ & -1.681 & 0.053 & -3.788 & 0.029 \\
$\alpha_{3,29}$ & -1.802 & 0.056 & -4.074 & 0.031 \\
$\alpha_{3,30}$ & -1.720 & 0.054 & -3.883 & 0.030 \\
\textbf{Covariate Coefficients} & & & &\\
$\beta_{1,1}$ & 0.072 & 0.007 & 0.109 & 0.005 \\
$\beta_{1,2}$ & 0.026 & 0.007 & 0.070 & 0.006 \\
$\beta_{1,3}$ & 0.095 & 0.006 & 0.120 & 0.005 \\
$\beta_{2,1}$ & 0.295 & 0.012 & 0.055 & 0.005 \\
$\beta_{2,2}$ & 0.204 & 0.013 & 0.073 & 0.007 \\
$\beta_{2,3}$ & 0.287 & 0.011 & 0.052 & 0.005 \\
$\beta_{3,1}$ & 0.303 & 0.012 & 0.036 & 0.004 \\
$\beta_{3,2}$ & 0.352 & 0.013 & 0.043 & 0.005 \\
$\beta_{3,3}$ & 0.276 & 0.011 & 0.037 & 0.003 \\
$\beta_{4,1}$ & 20.133 & 18.792 & 86.541 & 19.597 \\
$\beta_{4,2}$ & 7.666 & 21.558 & 51.860 & 22.202 \\
$\beta_{4,3}$ & 13.771 & 15.786 & 82.658 & 16.963 \\
\textbf{Hyperparameters} & & & & \\
$1/\sigma^2_1$ & 15.542 & 0.156 & 10.891 & 0.124 \\
$1/\sigma^2_2$ & 10.114 & 0.100 & 7.347 & 0.081 \\
$1/\sigma^2_3$ & 20.584 & 0.180 & 13.053 & 0.152 \\
$\rho_{12}$ & 0.567 & 0.004 & 0.661 & 0.004 \\
$\rho_{13}$ & 0.778 & 0.003 & 0.834 & 0.003 \\
$\rho_{23}$ & 0.775 & 0.003 & 0.818 & 0.003 \\
$\phi_{11}$ & 0.682 & 0.018 & 0.993 & 0.000 \\
$\phi_{21}$ & 0.331 & 0.022 &  &  \\
$\phi_{31}$ & 0.363 & 0.017 &  &  \\
$\phi_{12}$ & 0.258 & 0.018 &  &  \\
$\phi_{22}$ & 0.395 & 0.023 & 0.993 & 0.001 \\
$\phi_{32}$ & 0.095 & 0.018 &  &  \\
$\phi_{13}$ & -0.053 & 0.020 &  &  \\
$\phi_{23}$ & 0.164 & 0.025 &  &  \\
$\phi_{33}$ & 0.346 & 0.020 & 0.995 & 0.000 \\
$1/W_{1}$ & 43.668 & 3.187 & 35.364 & 2.234 \\
$1/W_{2}$ & 33.978 & 2.495 & 44.066 & 3.098 \\
$1/W_{3}$ & 48.089 & 3.394 & 40.906 & 2.539 \\
\end{longtable}
\end{center}


\begin{table}[H]\label{Table: LCM2}
\caption{Posterior Estimates for LCM2-VAR and LCM2-AR for Stock Market Index Data}
\label{Table-LCM2}
\fontsize{8}{10}\selectfont
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\cline{2-5}
\multicolumn{1}{c|}{\textbf{}} & \multicolumn{2}{c|}{\textbf{LCM2-VAR}} & \multicolumn{2}{c|}{\textbf{LCM2-AR}} \\ \hline
\multicolumn{1}{|c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{Posterior Mean}} & \multicolumn{1}{c|}{\textbf{Posterior SD}} & \multicolumn{1}{c|}{\textbf{Posterior Mean}} & \multicolumn{1}{c|}{\textbf{Posterior SD}} \\ \hline
\textbf{Component specific intercept} & & & & \\ 
$\alpha_{1}$ & -0.733 & 0.061 & -3.255 & 0.030 \\
$\alpha_{2}$ & -1.011 & 0.066 & -3.232 & 0.033 \\
$\alpha_{3}$ & -0.754 & 0.054 & -3.010 & 0.026 \\
\textbf{Covariate Coefficients} & & & & \\ 
$\beta_{1,1}$ & 0.087 & 0.007 & 0.238 & 0.006 \\
$\beta_{1,2}$ & 0.034 & 0.007 & 0.154 & 0.007 \\
$\beta_{1,3}$ & 0.107 & 0.006 & 0.235 & 0.006 \\
$\beta_{2,1}$ & 0.353 & 0.012 & 0.138 & 0.006 \\
$\beta_{2,2}$ & 0.246 & 0.013 & 0.167 & 0.007 \\
$\beta_{2,3}$ & 0.328 & 0.011 & 0.138 & 0.006 \\
$\beta_{3,1}$ & 0.442 & 0.011 & 0.041 & 0.004 \\
$\beta_{3,2}$ & 0.539 & 0.013 & 0.046 & 0.004 \\
$\beta_{3,3}$ & 0.430 & 0.010 & 0.043 & 0.003 \\
$\beta_{4,1}$& 12.616 & 18.798 & 70.801 & 20.368 \\
$\beta_{4,2}$ & -7.697 & 21.548 & 31.889 & 22.412 \\
$\beta_{4,3}$ & 2.042 & 15.798 & 64.558 & 17.541 \\
\textbf{Hyperparameter} & & & & \\ 
$1/\sigma_1^2$ & 15.784 & 0.207 & 8.623 & 0.104 \\
$1/\sigma_2^2$ & 10.218 & 0.132 & 6.457 & 0.080 \\
$1/\sigma_2^2$ & 21.161 & 0.321 & 10.470 & 0.134 \\
$\rho_{12}$ & 0.566 & 0.007 & 0.674 & 0.004 \\
$\rho_{13}$ & 0.786 & 0.007 & 0.842 & 0.002 \\
$\rho_{23}$ & 0.784 & 0.006 & 0.825 & 0.002 \\
$\phi_{11}$ & 0.462 & 0.147 & 0.995 & 0.000 \\
$\phi_{21}$ & 0.401 & 0.173 &  &  \\
$\phi_{31}$ & 0.462 & 0.136 &  &  \\
$\phi_{12}$ & 0.223 & 0.061 &  &  \\
$\phi_{22}$ & 0.441 & 0.088 & 0.995 & 0.001 \\
$\phi_{32}$ & 0.160 & 0.060 &  &  \\
$\phi_{13}$ & 0.264 & 0.175 &  &  \\
$\phi_{23}$ & 0.097 & 0.195 &  &  \\
$\phi_{33}$ & 0.185 & 0.157 & 0.995 & 0.000 \\
$1/W_{1}$ & 32.497 & 2.401 & 90.812 & 9.364 \\
$1/W_{2}$ & 27.300 & 2.087 & 60.335 & 5.854 \\
$1/W_{3}$ & 38.398 & 2.817 & 106.465 & 11.159\\ 
\hline
\end{tabular}
\end{center}
\end{table}

\subsection{Model Comparison}

We will make a comparison (in-sample) among the four models that we fitted . Bayesian model comparison in \texttt{R-INLA} is facilitated by the Deviance Information Criterion (DIC) \citep{spiegelhalter2002bayesian} and Watanabe-Akaike Information Criterion (WAIC) \citep{watanabe2010asymptotic}.

DIC is defined as
$$
DIC=-2 \log p\left(\boldsymbol{y}^{T} \mid \hat{\boldsymbol{x}}_{t, \text { Bayes }}\right)+2 p_{D I C}
$$
where $\hat{\boldsymbol{x}}_{t, \text { Bayes }}$ is the posterior mean of parameter $\boldsymbol{x}_{t}$ given the data $\boldsymbol{y}^{T}$ and $p_{D I C}$ is the effective number of parameters, defined as
$$
p_{DIC}=2\left(\log p\left(\boldsymbol{y}^{T} \mid \hat{\boldsymbol{x}}_{t, \text { Bayes }}\right)-E_{\text {post }}\left(\log p\left(\boldsymbol{y}^{T} \mid \boldsymbol{x}_{t}\right)\right)\right)
$$

where the expectation in the second term is an average of $\boldsymbol{x}_{t}$ over its posterior distribution.
WAIC is defined as
$$
\mathrm{WAIC}=\text{lppd} + p_{\mathrm{WAIC}}
$$
where lppd is the log pointwise posterior density given by
$$
\operatorname{lppd} =\sum_{t=1}^{T} \log \int p\left(y_{t} \mid \boldsymbol{x}_{t}\right) \pi\left(\boldsymbol{x}_{t} \mid \boldsymbol{y}^{T}\right) d \boldsymbol{x}_{t}
$$
and evaluated using draws $\boldsymbol{x}_{t}^{s}, s=1, \ldots, S$ from the posterior distribution of $\boldsymbol{x}_{t}$ as
$$
\sum_{t=1}^{T} \log \left(\frac{1}{S} \sum_{s=1}^{S} p\left(y_{t} \mid \boldsymbol{x}_{t}^{s}\right)\right)
$$
$p_{\text {WAIC }}$ is a correction term for the effective number of parameters to adjust for overfitting,
$$
p_{\mathrm{WAIC}}=2 \sum_{t=1}^{T}\left(\log \left(E_{\text {post }} p\left(y_{t} \mid \boldsymbol{x}_{t}\right)\right)-E_{\text {post }}\left(\log p\left(y_{t} \mid \boldsymbol{x}_{t}\right)\right)\right)
$$
and can be computed from draws $\boldsymbol{x}_{t}^{s}, s=1, \ldots, S$ as
$$
2 \sum_{t=1}^{T}\left(\log \left(\frac{1}{S} \sum_{s=1}^{S} p\left(y_{t} \mid \boldsymbol{x}_{t}^{s}\right)\right)-\frac{1}{S} \sum_{s=1}^{S} \log p\left(y_{t} \mid \boldsymbol{x}_{t}^{s}\right)\right)
$$

\begin{table}[H]
\begin{center}
\caption{Model Comparison}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Model} & \textbf{DIC} & \textbf{WAIC} \\ \hline
LCM1-AR & -593177.80 & -610362.30   \\ \hline
LCM1-VAR & -588168.80 & -598205.60  \\ \hline
LCM2-AR & -618968.40 & -628890.30   \\ \hline
LCM2-VAR & -570362.80 & -578713.10   \\ \hline
\end{tabular}
\end{center}
\end{table}

The lowest DIC and WAIC is obtained by LCM2-AR and hence LCM2-AR is the best model by this criteria. We note that according to DIC and WAIC, the AR counterparts are better than VAR. This shows that LCM1-VAR and LCM2-VAR do not fit the data appreciably better than LCM1-AR and LCM1-VAR respectively.
